Multi-modal Contrastive Representation Learning for Entity Alignment

Multi-modal entity alignment aims to identify equivalent entities between two different multi-modal knowledge graphs, which consist of structural triples and images associated with entities. Most previous works focus on how to utilize and encode information from different modalities, while it is not trivial to leverage multi-modal knowledge in entity alignment because of the modality heterogeneity. In this paper, we propose MCLEA, a Multi-modal Contrastive Learning based Entity Alignment model, to obtain effective joint representations for multi-modal entity alignment. Different from previous works, MCLEA considers task-oriented modality and models the inter-modal relationships for each entity representation. In particular, MCLEA firstly learns multiple individual representations from multiple modalities, and then performs contrastive learning to jointly model intra-modal and inter-modal interactions. Extensive experimental results show that MCLEA outperforms state-of-the-art baselines on public datasets under both supervised and unsupervised settings.

==> sections/abstract.tex <==
\begin{abstract}
Multi-modal Information could depict different aspects of entities and alleviate the long-tail problem, which plays an increasingly important role in entity alignment.
In this paper, we propose a multi-modal contrastive representation learning framework (MuCRL) to learn entity representations from multi-modal knowledge graphs for entity alignment.
MuCRL firstly learns multiple separate representations from multiple modalities based on respective encoders, and performs contrastive learning to model intra-modal and inter-modal relations.
MuCRL chooses a multi-task learning paradigm to learn intra-modal representations and inter-modal relations jointly. Besides, MuCRL applies task-dependent uncertainty to adaptively tune the loss weights of tasks during training.

\end{abstract}

==> sections/experiment.tex <==
\section{Experiments}

\subsection{Experimental Setup}
\noindent\textbf{Datasets}.
Five EA datasets are adopted for evaluation, including three bilingual datasets ZH/JA/FR-EN versions of DBP15K~\cite{liu2021visual} and two cross-KG datasets FB15K-DB15K/YAGO15K~\cite{chen2020mmea}.
The detailed dataset statistics are listed in Table~\ref{tab:dataset} where ``DBP15K" and ``-15K" are omitted.
Note that not all entities have corresponding images and for those without images, MCLEA would assign random vectors for the visual modality, as the setting of EVA~\cite{liu2021visual}.
% As for DBP15K, each dataset provides 30\% entities as ``seed alignments'' by default and leaves the remaining for evaluating EA performance. As for cross-KG datasets, following ~\cite{chen2020mmea}, each dataset provides 20\%, 50\%, and 80\% reference entity alignment as training sets, respectively.
As for DBP15K datasets, 30\% reference entity alignment are given as ``seed alignments" while as for cross-KG datasets, 20\%, 50\%, and 80\% reference entity alignment are given~\cite{chen2020mmea}.

\noindent\textbf{Baselines}.
% we compare MCLEA against state-of-the-art baselines in entity alignment, including three types of models.
We compare the proposed MCLEA against a total of 14 state-of-the-art EA methods. These methods can be classified into four categories:
1) \textit{structure-based methods} that solely rely on structural information for aligning entities, including MUGNN~\cite{cao2019multi}, KECG~\cite{li2019semi}, BootEA~\cite{sun2018bootstrapping}, NAEA~\cite{zhu2019neighborhood}, and AliNet~\cite{sun2020knowledge};
2) \textit{auxiliary-enhanced methods} that utilize auxiliary information (e.g., attribute or surface form) to improve the performance, including MultiKE~\cite{zhang2019multi}, HMAN~\cite{yang2019aligning}, RDGCN~\cite{wu2019relation}, AttrGNN~\cite{liu2020exploring}, and BERT-INT~\cite{tang2021bert};
3) \textit{multi-modal methods} that combine the multi-modal features to generate entity representations, including PoE~\cite{liu2019mmkg}, MMEA~\cite{chen2020mmea}, and EVA~\cite{liu2021visual};
4) \textit{unsupervised methods}, including MRAEA~\cite{mao2020mraea}, EASY~\cite{ge2021make}, and SEU~\cite{mao2021alignment}.

\noindent\textbf{Implementation Details}.
% If entities’ names are in different languages in two KGs, following previous work~\cite{xu2019cross}, we use machine translation tool to translate names in non-English language to English language.
% For bilingual DBP15K, we use machine translation tool to translate entity names from both languages into the same language.
The hidden size of each layer of GAT is 300, while the embedding size of the other modalities is 100. We use AdamW optimizer with a learning rate of $5e-4$ to update the parameters. The number of training epochs is 1000 with early-stopping and the batch size is 512. The hyper-parameters $\tau_1, \tau_2$ are set to 0.1 and 4.0, respectively. 
% To make fair comparisons with previous work, we use the same entity name translations and word vectors provided by~\cite{xu2019cross} for bilingual datasets.
For fair comparisons, we also use the same entity name translations and word vectors provided by~\cite{xu2019cross} for bilingual datasets.
For visual embedding, we adopt the preprocessed image features provided by~\cite{liu2021visual} and~\cite{chen2020mmea} for bilingual datasets and cross-KG datasets, where the former uses ResNet-152~\cite{he2016deep} as the pre-trained backbone, while the latter uses VGG-16~\cite{simonyan2014very}.
For the unsupervised setting, we implement two variants, MCLEA-V and MCLEA-N, which generate pseudo-alignment seeds based on the similarities of images and names, respectively.

\begin{table}[ht]
    \centering
    \scriptsize
    \caption{Dataset Statistics.}
    \begin{tabular}{@{}l|l|rrrrrrr@{}}
        \toprule
        Dataset & KG & \#Ent. & \#Rel. & \#Attr. & \#Rel tr. & \#Attr tr. & \#Image \\
        \midrule
        \multirow{2}*{ZH-EN} & ZH & 19,388 & 1,701 & 8,111 & 70,414 & 248,035 & 15,912 \\
        & EN & 19,572 & 1,323 & 7,173 & 95,142 & 343,218 & 14,125 \\
        \midrule
        \multirow{2}*{JA-EN} & JA & 19,814 & 1,299 & 5,882 & 77,214 & 248,991 & 12,739 \\
        & EN & 19,780 & 1,153 & 6,066 & 93,484 & 320,616 & 13,741 \\
        \midrule
        \multirow{2}*{FR-EN} & FR & 19,661 & 903 & 4,547 & 105,998 & 273,825 & 14,174 \\
        & EN & 19,993 & 1,208 & 6,422 & 115,722 & 351,094 & 13,858 \\
        \midrule
        \multirow{2}*{FB-DB} & FB & 14,951 & 1,345 & 116 & 592,213 & 29,395 & 13,444 \\
        & DB & 12,842 & 279 & 225 & 89,197 & 48,080 & 12,837 \\
        \midrule
        \multirow{2}*{FB-YG} & FB & 14,951 & 1,345 & 116 & 592,213 & 29,395 & 13,444 \\
        & YG & 15,404 & 32 & 7 & 122,886 & 23,532 & 11,194 \\
        \bottomrule
    \end{tabular}
    \label{tab:dataset}
\end{table}

\noindent\textbf{Evaluation}.
Following the convention~\cite{liu2021visual}, we rank matching candidates of each to-be-aligned entity and use the metrics of Hits@1 (H@1), Hits@10 (H@10), and mean reciprocal rank (MRR).
In the following tables, the best results are \textbf{in bold} with the second best results \underline{underlined}.

\begin{table*}[ht]
    \centering
    \footnotesize
    \caption{Experimental results on three bilingual datasets where sup./unsup. denote the supervised/unsupervised settings.}
    \begin{tabular}{@{}l|l|ccc|ccc|ccc@{}}
        \toprule
        & \multirow{2}*{Models} & \multicolumn{3}{c|}{DBP15K$_{ZH-EN}$} & \multicolumn{3}{c|}{DBP15K$_{JA-EN}$} & \multicolumn{3}{c}{DBP15K$_{FR-EN}$} \\
        & & {\scriptsize H@1} & {\scriptsize H@10} & {\scriptsize MRR} & {\scriptsize H@1} & {\scriptsize H@10} & {\scriptsize MRR} & {\scriptsize H@1} & {\scriptsize H@10} & {\scriptsize MRR} \\
        \midrule
        % & MTransE {\scriptsize \cite{chen2016multilingual}} & 
        % .224 & .556 & .335 & .279 & .575 & .349 & .308 & .614 & .364 \\
        % & GCN-Align {\scriptsize \cite{wang2018cross}} & 
        % .373 & .745 & .532 & .399 & .745 & .546 & .413 & .744 & .549 \\
        \parbox[t]{2mm}{\multirow{12}{*}{\rotatebox[origin=c]{90}{sup.}}} & MUGNN {\scriptsize \cite{cao2019multi}} & 
        .494 & .844 & .611 &  .501 & .857 & .621 & .495 & .870 & .621\\
        & KECG {\scriptsize \cite{li2019semi}} & 
        .478 & .835 & .598 & .490 & .844 & .610 & .486 & .851 & .610\\
        & BootEA {\scriptsize \cite{sun2018bootstrapping}} & 
        .629 & .847 & .703 & .622 & .854 & .701 & .653 & .874 & .731 \\
        & NAEA {\scriptsize \cite{zhu2019neighborhood}} & 
        .650 & .867 & .720 & .641 & .873 & .718 & .673 & .894 & .752 \\
        & AliNet {\scriptsize \cite{sun2020knowledge}} & 
        .539 & .826 & .628 & .549 & .831 & .645 & .552 & .852 & .657 \\
        % \cmidrule(lr){2-11}
        & MultiKE {\scriptsize \cite{zhang2019multi}} & 
        .437 & .516 & .466 & .570 & .643 & .596 & .714 & .761 & .733 \\
        & HMAN {\scriptsize \cite{yang2019aligning}} & 
        .562 & .851 & -- & .567 & .969 & -- & .540 & .871 & -- \\
        & RDGCN {\scriptsize \cite{wu2019relation}} & 
        .708 & .846 & -- & .767 & .895 & -- & .886 & .957 & -- \\
        & AttrGNN {\scriptsize \cite{liu2020exploring}} & 
        .777 & .920 & .829 & .763 & .909 & .816 & .942 & .987 & .959 \\
        & BERT-INT {\scriptsize \cite{tang2021bert}} & 
        \underline{.968} & \underline{.990} & \underline{.977} & \underline{.964} & \underline{.991} & \underline{.975} & \underline{.992} & \underline{.998} & \underline{.995}\\
        % \cmidrule(lr){2-11}
        & EVA {\scriptsize \cite{liu2021visual}} & 
        .761 & .907 & .814 & .762 & .913 & .817 & .793 & .942 & .847 \\
        \cmidrule(lr){2-11}
        & \textbf{MCLEA} {\scriptsize (Ours)} & 
        \textbf{.972} & \textbf{.996} & \textbf{.981} & \textbf{.986} & \textbf{.999} & \textbf{.991} & \textbf{.997} & \textbf{1.00} & \textbf{.998} \\
        \midrule
        \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{unsup.}}} & MRAEA {\scriptsize \cite{mao2020mraea}} & 
        .778 & .832 & -- & .889 & .927 & -- & .950 & .970 & -- \\
        & EASY {\scriptsize \cite{ge2021make}} & 
        .898 & \underline{.979} & \underline{.930} & .943 & .990 & .960 & .980 & .998 & .990 \\
        & SEU {\scriptsize \cite{mao2021alignment}} & 
        \underline{.900} & .965 & .924 & \underline{.956} & \underline{.991} & \underline{.969} &  \underline{.988} & \underline{.999} & \underline{.992}\\
        \cmidrule(lr){2-11}
        & \textbf{MCLEA-V} {\scriptsize (Ours)} & 
        .959 & \textbf{.995} & \textbf{.974} & .977 & \textbf{.999} & .987 & .990 & \textbf{1.00} & .994 \\
        & \textbf{MCLEA-N} {\scriptsize (Ours)} & \textbf{.960} & 
        .994 & \textbf{.974} & \textbf{.983} & \textbf{.999} & \textbf{.990} & \textbf{.995} & \textbf{1.00} & \textbf{.997} \\
        \bottomrule
    \end{tabular}
    \label{tab:overall-perf-1}
\end{table*}

\subsection{Overall Results}

\begin{table}[ht]
    \centering
    \scriptsize
    \caption{Experimental results on two cross-KG datasets where X\% represents the percentage of ground-truth entity alignment used as training sets. The symbol $\ast$ denotes the reproduced results based on the published source code, and $\dagger$ denotes an MCLEA variant without name embedding.}
    \begin{tabular}{@{}l|l|ccc|ccc@{}}
        \toprule
        & \multirow{2}*{Models} & \multicolumn{3}{c|}{FB15K-DBP15K} & \multicolumn{3}{c}{FB15K-YAGO15K} \\
        & & {\tiny H@1} & {\tiny H@10} & {\tiny MRR} & {\tiny H@1} & {\tiny H@10} & {\tiny MRR} \\
        \midrule
        \parbox[t]{1mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{20\%}}} & PoE  & 
        .126 & .251 & .170 & .113 & .229 & .154 \\
        & MMEA & \underline{.265} & \underline{.541} & \underline{.357} & \underline{.234} & \underline{.480} & \underline{.317} \\
        & EVA$\ast$ & .134 & .338 & .201 & .098 & .276 & .158 \\
        & \textbf{MCLEA}$\dagger$ & .445 & .705 & .534 & .388 & .641 & .474 \\
        & \textbf{MCLEA} & \textbf{.992} & \textbf{.998} & \textbf{.995} & \textbf{.992} & \textbf{.996} & \textbf{.994} \\
        \midrule
        \parbox[t]{1mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{50\%}}} & PoE & 
        \underline{.464} & .658 & \underline{.533} & .347 & .536 & .414 \\
        & MMEA & .417 & \underline{.703} & .512 & \underline{.403} & \underline{.645} & \underline{.486} \\
        & EVA$\ast$ & .223 & .471 & .307 & .240 & .477 & .321 \\
        & \textbf{MCLEA}$\dagger$ & .573 & .800 & .652 & .543 & .759 & .616 \\
        & \textbf{MCLEA} & \textbf{.993} & \textbf{.998} & \textbf{.995} & \textbf{.994} & \textbf{.998} & \textbf{.995} \\
        \midrule
        \parbox[t]{1mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{80\%}}} & PoE  & 
        \underline{.666} & .820 & \underline{.721} & .573 & .746 & .635 \\
        & MMEA & .590 & \underline{.869} & .685 & \underline{.598} & \underline{.839} & \underline{.682} \\
        & EVA$\ast$ & .370 & .585 & .444 & .394 & .613 & .471 \\
        & \textbf{MCLEA}$\dagger$ & .730 & .883 & .784 & .653 & .835 & .715 \\
        & \textbf{MCLEA} & \textbf{.996} & \textbf{.999} & \textbf{.997} & \textbf{.995} & \textbf{.997} & \textbf{.996} \\
        \bottomrule
    \end{tabular}
    \label{tab:overall-perf-2}
\end{table}

% Table \ref{tab:overall-perf-1} and \ref{tab:overall-perf-2} report the performance of our approaches against other methods on bilingual and cross-KG datasets.
\noindent\textbf{Supervised EA}. As reported in Table~\ref{tab:overall-perf-1} on bilingual datasets, it is observed that MCLEA outperforms the state-of-the-art results on all bilingual datasets. Firstly, compared with the first group that purely relies on structure information, MCLEA brings about XX\%$\sim$XX\% absolute improvement in H@1 over the best baseline.
The superiority of MCLEA confirms that employing multiple modalities substantially promotes the EA results.
Compared with the second group with auxiliary information involvement, MCLEA still gains about XX\%$\sim$XX\% absolute improvement in H@1 over the best baseline BERT-INT.
It is worth mentioning that BERT-INT directly fine-tunes a multi-lingual BERT as the backbone whose parameters are several magnitudes larger than MCLEA (110M $vs.$ XX).
On the other hand, MCLEA outperforms the multi-modal method EVA by XX\%, XX\% and XX\% in H@1 on FR-EN, JA-EN and ZH-EN respectively. It is contributed by two reasons. 
First, MCLEA utilizes more abundant modal features, such as entity names, to provide a more comprehensive entity representation for EA.
Second, MCLEA devises ICL and IAL to sufficiently capture the dynamics within and between modalities while preserving semantic proximity and minimizing the modality gap.

Notably, in table \ref{tab:overall-perf-2}, MCLEA advances the H@1 to above 99\% on all cross-KG datasets, even with only 20\% of training seeds. The reason is that entity names in Freebase, DBpedia and YAGO are nearly identical, making the name features very effective.
To further illustrate the effectiveness of our model, we introduce a variant that removes the name embedding, corresponding to ``MCLEA w/o name'' in Table \ref{tab:overall-perf-2}.
Even the name embedding is removing, MCLEA still gains about XX\%$\sim$XX\% absolute improvement in H@1 over the best baseline cross different ratio of seeds.
The fact that a simple name feature can achieve strong performance on current benchmarks also encourages us to build more challenging cross-KG EA datasets, which is left for future work.

\noindent\textbf{Unsupervised EA}. 
To demonstrate the flexibility of MCLEA, we provide two variants, namely MCLEA-V and MCLEA-N, which generate pseudo training seeds based on image similarities and name similarities respectively.
Even unsupervised setting, MCLEA still achieves satisfactory results.

\todo{
Table \ref{tab:overall-perf-1} and \ref{tab:overall-perf-2} report the performance of MCLEA against other baselines on bilingual and cross-KG datasets, respectively.
Overall, MCLEA and its variants perform the best across all the datasets on all the metrics.

As shown in Table~\ref{tab:overall-perf-1}, we find that, in the supervised setting, MCLEA greatly outperforms all the structure-based, auxiliary-enhanced, and multi-modal methods except BERT-INT by a large margin from 5\% to 20\% in H@1.
BERT-INT achieves near-perfect scores as it directly fine-tunes a multi-lingual BERT as the backbone; MCLEA shows comparable performance to BERT-INT but with far less parameters (110M $vs.$ XXX).
When compared to the unsupervised methods, both variants of MCLEA perform slightly better than the best baseline SEU, and for instance, the performance gain in H@1 varies from 0.7\% to 6.7\%.

Table~\ref{tab:overall-perf-2} shows the comparison of multi-modal methods on two cross-KG datasets, which provides direct evidence of the effectiveness of MCLEA.
When 20\% alignment seeds are given for training, MCLEA outperforms the best baseline MMEA with more than 270\% higher in H@1, 80\% higher in H@10, and 170\% higher in MRR.
For the variant MCLEA$\dagger$ which rules out the most discriminative feature, the performance gains are still obvious with more than 60\% in H@1, 30\% in H@10, and 40\% in MRR.
Similar findings are also observed when 50\% and 80\% alignment seeds are given.
It is worthy noting that the performance gains reach the highest in the 20\% setting, indicating that MCLEA could fully utilize the minimum amount of alignment seeds to obtain effective representations.
}

\subsection{Ablation Studies}

We perform ablation study to gain insights into the components of MCLEA. The result on $\text{DBP15K}_{ZH-EN}$ and $\text{DBP15K}_{JA-EN}$ are presented in Table~\ref{tab:ablation}.
We first examine the contribution of different modality features. As can be observed from Table~\ref{tab:ablation} that the removal of each modality has varying degrees of negative impact on performance. Firstly, removing structural information significantly
brings performance drop, showing its stable effectiveness across different datasets.
% In comparison, pruning relation or visual information does not hurt the accuracy too much. 
In comparison, relations, attributes or visual information give minor but consistent improvement to all metrics.
Specially, surface form (etc. entity name) plays an important role and pruning it results in considerable accuracy drop. This is in line with the findings by~\cite{wu2019relation,mao2020mraea,ge2021make}. This unveils that name feature is quite useful on datasets where entity names are similar.
Notably, even without the surface form, MCLEA still outperforms some auxiliary-enhanced methods whose use surface form, such as HMAN, RDGCN and AttrGNN.


Furthermore, we test inspect the importance of various training strategies.
From the experimental result, it can be seen that removing the ICL (i.e., removing the second term in Eq.~(\ref{eq:loss2})) dramatically degrades the performance.
It indicates that the learning of intra-modal proximity is the fundamental component that leads to the high performance of our model.
Without the IAL (i.e., removing the third term in Eq.~(\ref{eq:loss2})) also hurts the performance, revealing the significance of considering the interdependence between different modalities.
Besides, iterative strategy is an effective tool to alleviate the inadequate prior alignment.
Finally, replacing the uncertainty mechanism with uniform weights (last row) causes slight drops in performance.
% Besides, replacing the uncertainty mechanism with uniform weights (row) causes slight drops in performance, showing the effectiveness of the adaptive loss weighting mechanism while avoiding manual tuning for multiple losses.
% We remark that the above components jointly contribute to the model performance, and removing any of them hurts the classification accuracy.
Overall, combining all the above components together enables our model to achieve the state-of-the-art.


% \noindent\textbf{Impact of different modalities}. 
% The results in Table \ref{tab:ablation} show that the removal of each modality has a negative impact on the performance.

% \noindent\textbf{Impact of different training strategies}.

\begin{table}[h!]
    \centering
    \scriptsize
    \caption{Ablation studies on bilingual datasets.}
    \begin{tabular}{@{}l|l|ccc|ccc@{}}
        \toprule
        & \multirow{2}*{Models} & \multicolumn{3}{c|}{DBP15K$_{ZH-EN}$} & \multicolumn{3}{c}{DBP15K$_{JA-EN}$} \\
        & & {\tiny H@1} & {\tiny H@10} & {\tiny MRR} & {\tiny H@1} & {\tiny H@10} & {\tiny MRR} \\
        \midrule
        & MCLEA & \textbf{.972} & \textbf{.996} & \textbf{.981} & \textbf{.986} & \textbf{.999} & \textbf{.991} \\
        \midrule
        \parbox[t]{1mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{features}}} 
        % & w/o char & .931 & .987 & .952 \\
        % & w/o name & .967 & .995 & .978 \\
        & w/o structure & .883 & .956 & .909 & .947 & .980 & .959 \\
        & w/o relation & .967 & .995 & .978 & .985 & .999 & .991 \\
        & w/o attribute & .961 & .994 & .974 & .983 & .999 & .991 \\
        & w/o name & .816 & .948 & .865 &  .812 & .952 & .865 \\
        & w/o visual & .968 & .994 & .978 & .985 & .999 & .991 \\
        \midrule
        \parbox[t]{1mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{training}}} 
        & w/o ICL & .782 & .892 & .818 & .813 & .909 & .844 \\
        & w/o IAL & .966 & .995 & .977 & .980 & .998 & .987 \\
        & w/o iterative strategy & .942 & .991 & .960 & .964 & .995 & .976 \\
        & w/o uncertainty & .969 & .996 & .980 & .984 & .999 & .990 \\
        \bottomrule
    \end{tabular}
    \label{tab:ablation}
\end{table}

\subsection{Model Analysis}

% \noindent\textbf{Unsupervised EA Implementation}.

\noindent\textbf{Impact of hypar-parameters $\tau_1, \tau_2$}.
We examine the effects of hyper-parameters $\tau_1$ and $\tau_2$ on the $\text{DBP15K}_{ZH-EN}$.
As shown in Figure~\ref{fig:params}, the choice of $\tau_1$ has drastic effects on the model, especially on H@1 and MRR. 
The is because the temperature $\tau_1$ controls the strength of penalties on hard negative samples~\cite{wang2021understanding}, an appropriate $\tau_1$ is conducive to learning a discriminative entity embedding.
Instead, $\tau_2$ has more robust effects, and the model performance reaches saturation when $\tau_2=4.0$.
% Using a higher $\tau_2$ produces a softer alignment distribution over entities.
$\tau_2$ regulates the softness of the alignment distribution produced by joint embedding, which can establish the associations between different modalities and transfer the generalization ability of the joint embedding to unimodal embedding.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{sections/pics/params.pdf}
    \caption{Impact of different $\tau_1, \tau_2$}
    \label{fig:params}
\end{figure}

==> sections/introduction.tex <==
\section{Introduction}

Knowledge Graphs (KGs) such as DBpedia~\cite{lehmann2015dbpedia} and YAGO~\cite{mahdisoltani2014yago3} store abundant structured knowledge that express relations of many concepts and real-world entities, which have been widely employed in various knowledge-driven applications like question answering~\cite{cui2017kbqa}, recommendation system~\cite{cao2019unifying}, and information extraction~\cite{han2018neural}.
% Most of the existing KGs are highly incomplete and independently constructed from different data sources but the knowledge is usually complementary to each other. 
Most of the existing KGs are highly incomplete but the knowledge is usually complementary to each other. 
% Therefore, integrating heterogeneous knowledge from different sources provides an effective way to enlarge the coverage of a unified knowledge graph. Entity Alignment (EA) seeks to discover identical entities from different KGs that refer to the same real-world objects.
Therefore, Entity Alignment (EA) techniques are urgently required to integrate heterogeneous knowledge from distinct KGs by linking entities that refer to the same real-world objects, which provides an effective way to enlarge the coverage of a unified KG.

Early studies for EA identify similar entities mostly focus on exploring the symbolic similarity, such as names~\cite{raimond2008automatic} and attribute values~\cite{volz2009discovering}.
However, these methods often fail to deal with the semantic heterogeneity between different KGs.
Recently, significant progress has been made in applying knowledge graph embedding representation for EA~\cite{wang2018cross,zhu2019neighborhood,sun2020knowledge}. These methods are usually based on the assumption that entities and their counterparts from other KGs have similar neighborhood. Concretely, they embed entities from different KGs into a unified low-dimensional vector space by translated-based model or graph neural network and find their counterparts according to the similarity of embeddings. Nevertheless, the assumption does not always hold for real-life scenarios because different KGs usually have heterogeneous schemas and data incompleteness~\cite{pujara2013knowledge}. To further improve the EA performance, many efforts have been devoted to exploit various auxiliary information, such as attribute values~\cite{trisedya2019entity,liu2020exploring,wang2020knowledge}, 
entity types~\cite{xiang2021ontoea} or descriptions~\cite{chen2018co,zhang2019multi,yang2019aligning,tang2021bert}. 
% However, the capabilities of existing EA methods are still limited and worthy of further exploration.
However, the capabilities of existing EA methods are still limited, yet without exploiting the full potential of multiple modalities for knowledge.

As a great deal of real-life knowledge can be expressed in multi-modal formats, visual modality of entities have received considerable attention in the field of KGs.
Images (e.g. profile photos, thumbnails, posters) are the most commonly used visual modality of entities~\cite{wang2021visual}, which describe the appearances and behaviours of corresponding entities. 
The images can help to enhance the contextual semantics of entities and provides an opportunity to enhance the performance of rare KG entities in the absence of structural information,  facilitating conventional KG-based applications such as knowledge completion~\cite{xie2017image}, entity linking~\cite{moon2018multimodal}, and so on.
% In recent years, multi-modal entity alignment has also received increasing attention from researchers.
Researchers have also paid increasing attention to multi-modal entity alignment in recent years.
The underlying idea is that images that correspond to aligned entities are usually semantically similar, which can serve as visual pivot for entity alignment.
The pioneer PoE~\cite{liu2019mmkg} combines the multi-modal features through extracting relational, numerical and visual information and measures the credibility of facts by matching the underlying semantics of the entities.
Furthermore, MMEA~\cite{chen2020mmea} and EVA~\cite{liu2021visual} design distinct multi-modal fusion modules to integrate knowledge representations from multiple modalities into a joint embedding.
The consensus reached by these methods is that multi-modal features (neighbor structure, attribute, image, etc.) characterize different aspects of entity identities, which provide additional redundancy for better robustness. However, the above methods mainly focus on exploring the use of diverse modality-specific features to enhance the contextual representation of entities, but neglect to the consider inter-modal relationships, which are also informative to help reach more discriminatory boundaries and narrow the modality gap.

The above observation motivates us to propose a unified Multi-modal Contrastive Learning Framework (abbr. MuCRL) to effectively integrate multi-modal information and learn a comprehensive entity embedding for EA. 
% Learning meaningful representation for multi-modal KGs is challenging because there exist distributional shift between different modalities. To address these challenges,
Specifically, MuCRL firstly utilizes different encoders to obtain modality-specific representations of entities for each modality, including neighborhood structure, relation, attribute, image and surface form.
Furthermore, we propose intra- and inter-modal loss objectives to learn a discriminative cross-modal latent embedding and ensure that entities with similar content stay close in the joint embedding space, regardless of the modality.

In summary, the contributions of this paper are as follows: 
% First, we propose a general representation learning framework that integrates multi-modal information of entities and simultaneously explores intra-modal relationships and learn cross-modal interactions to obtain high-quality representations of entities for entity alignment.
First, we propose a general representation learning framework that embeds different modalities into a unified vector space and obtains high-quality representations of entities based on latest contrastive learning for entity alignment.
% Second, considering inter-modal relationships that are neglected in existing EA work, two novel ways of contrastive learning are devised to train the model, i.e., IAMCL, IEMCL and SCL.
Second, we elaborately devise two novel losses to explore intra-modal relationships and learn cross-modal interactions, ensuring that aligned entities between different KGs are pulled closer than those that are not aligned in the feature space.
Third, our proposed MuCRL is compared with several models on public datasets and achieves state-of-the-art performance even with very simple fusion methods, which demonstrates its effectiveness and superiority. The overall results suggest that our MuCRL can learn a more discriminative embedding space for entity alignment.

==> sections/work.tex <==
\section{Related Work}

\subsection{Entity Alignment}

With the rapid development of contextualized representations, deep embedding-based EA models are superior to the traditional symbolic-based models due to its flexibility and effectiveness.

However, the existing researches mainly focus on the alignment of semantic or conceptual knowledge graphs, but largely neglect to the multi-modal knowledge from the real scenarios.
Integrating multiple modalities is beneficial to provide useful clues from different perspectives for entity alignment.

\subsection{Multi-modal Knowledge Graph}

PoE is proposed to find entity alignment in multi-modal knowledge graphs through extracting relational, latent, numerical and visual features.
PoE combines the multi-modal features and measures the credibility of facts by matching the underlying semantics of the entities and mining the relations contained in the embedding space.

IKRL integrates image representations into an aggregated image-based representation via an attention-based method.

MKBE models knowledge bases that contain a variety of multi-modal features such as links, images, numerical and categorical values. It applies neural encoders and decoders which embed multi-modal evidence types and generate multi-modal attributes, respectively. [8] proposes a multi-modal translation-based method, which defines the energy of a knowledge graph triple as the sum of sub-energy functions that leverages structural, visual and linguistic knowledge representations.

[EVA] Through an attention-based modality weighting scheme, we fuse multi-modal information from KGs into a joint embedding and allow the alignment model to automatically adjust modality weights.

[mmea] Moreover, a multi-modal fusion method was designed through common space learning to migrate features under different knowledge spaces.

The above approaches mostly focus on learning joint representations in a common manifold, using plain fusion module to obtain cross-modal interactions for better performance. However, they cannot ensure to align modalities well with each other and still suffer modality gap.
% More importantly, the above methods mainly focus on exploring the use of diverse modality-specific features to enhance the contextual representation of entities, but neglect to the consider inter-modal relationships, which are also informative to help reach more discriminatory boundaries and narrow the modality gap.

Despite the simplicity of the fusion method, our proposed model still obtains new state-of-the-art results.

{\color{red}{the difference with others}}
Unlike previous work that rely on fusion module to interact with different modal features, MuCRL allow to learn intra-/inter-modal dynamics simultaneously.

In this paper, we propose a general framework that can support unlimited number of modalities of KG.

